Autoencoding Conditional Neural Processes for Representation Learning

Conditional neural processes (CNPs) are a flexible and efficient family of models that learn to learn a stochastic process from data. They have seen particular application in contextual image completion - observing pixel values at some locations to predict a distribution over values at other unobserved locations. However, the choice of pixels in learning CNPs is typically either random or derived from a simple statistical measure (e.g. pixel variance). Here, we turn the problem on its head and ask: which pixels would a CNP like to observe - do they facilitate fitting better CNPs, and do such pixels tell us something meaningful about the underlying image? To this end we develop the Partial Pixel Space Variational Autoencoder (PPS-VAE), an amortised variational framework that casts CNP context as latent variables learnt simultaneously with the CNP. We evaluate PPS-VAE over a number of tasks across different visual data, and find that not only can it facilitate better-fit CNPs, but also that the spatial arrangement and values meaningfully characterise image information - evaluated through the lens of classification on both within and out-of-data distributions. Our model additionally allows for dynamic adaption of context-set size and the ability to scale-up to larger images, providing a promising avenue to explore learning meaningful and effective visual representations.

==> content/conclusion.tex <==
\section{Conclusion}
%
We present \ppsvae, a novel VAE framework that allows us to infer context set/PPS for conditional neural processes (CNPs).
%
We formulate our model and evaluate it across multiple vision datasets, while exploring the utility of learning context sets in both unsupervised and supervised manner.
%
First, we show that the learning distribution over PPS results in better models for images.
%
Then, we observe that with the appropriate inductive biases and latent variables, the model is able to induce context sets that are visually meaningful. We validate this observation quantitatively through the lens of classification.
%
On the classification tasks, \ppsvae\ achieves superior performance against the baselines and PPS resulting in better features for a classifier than an original image is on the CLEVR dataset indicating that the framework has promise as a model for learning meaningful representations of data. Moreover, we test our model on the same classification tasks but in out-of-distribution settings showing that it can infer PPS that generalises to an out-of-distribution datasets. Finally, we show a differentiating property of PPS-VAE --- an ability to change the capacity of PPS at inference time.



==> content/limitations.tex <==
\section{Limitations}
We would like to outline a number of limitation the present framework has: 
\begin{compactitem}
    \item Presently we provide an observatory analysis of the induced context set an put forward hypothesis regarding types of points the model learns. However, human level interpretability of the context set is limited. To improve it, instead of inferring a single location, a more interpretable encoder could capture M ‘closed’ regions. This would allow us to compare against the slot-attention models such as \citet{locatello2020objectcentric}.
    \item Exploration of inductive biases, and modelling updates would be interesting avenues to see if the latent variable can capture relevant information more cleanly.
    \item Presently we fix $M$ to a certain value and provide analysis for its various values. However, it may be limiting to decide on the value of $M$ beforehand because we do not know what value would be optimal for each image in a dataset. Allowing the model to decide on the value of $M$ during the learning based on dataset may solve this issue.
\end{compactitem}

\section{Broader Impacts}
The work we describe in this paper aims to improve the interpretability of the latent representations. We foresee that further development of the described algorithm  may allow 
 to overcome a number of drawbacks of Deep Generative Models (DGMs) e.g. \citet{feng2023trainingfree, conwell2022testing} by addressing these issues at the representation level (e.g. by explicit manipulation of latent representations to rectify mistakes DGMs). However, the current work is  algorithmic in nature. And at present stage is not tied to particular applications, let alone deployments.
